The New Small Wheel electronics

The increase in luminosity, and consequent higher backgrounds, of the LHC upgrades require improved rejection of fake tracks in the forward region of the ATLAS Muon Spectrometer. The New Small Wheel upgrade of the Muon Spectrometer aims to reduce the large background of fake triggers from track segments that are not originated from the interaction point. The New Small Wheel employs two detector technologies, the resistive strip Micromegas detectors and the "small" Thin Gap Chambers, with a total of 2.45 Million electrodes to be sensed. The two technologies require the design of a complex electronics system given that it consists of two different detector technologies and is required to provide both precision readout and a fast trigger. It will operate in a high background radiation region up to about 20 kHz/cm$^{2}$ at the expected HL-LHC luminosity of $\mathcal{L}$=7.5$\times10^{34}$cm$^{-2}$s$^{-1}$. The architecture of the system is strongly defined by the GBTx data aggregation ASIC, the newly-introduced FELIX data router and the software based data handler of the ATLAS detector. The electronics complex of this new detector was designed and developed in the last ten years and consists of multiple radiation tolerant Application Specific Integrated Circuits, multiple front-end boards, dense boards with FPGA's and purpose-built Trigger Processor boards within the ATCA standard. The New Small Wheel has been installed in 2021 and is undergoing integration within ATLAS for LHC Run 3. It should operate through the end of Run 4 (December 2032). In this manuscript, the overall design of the New Small Wheel electronics is presented.

==> sections/authors.tex <==
 \author[a,1]{George Iakovidis \note{Corresponding author}}
 \author[b,1]{Lorne Levinson}
 \affiliation[a]{Brookhaven National Laboratory}
 \affiliation[b]{Weizmann Institute of Science}


% e-mail addresses: only for the corresponding author
\emailAdd{giakovidis@bnl.gov}
\emailAdd{lorne.levinson@weizmann.ac.il}


==> sections/todo.tex <==

\section{\red{To do}}
\red{\\
Global changes for consistency:
\begin{itemize}[topsep=2pt, itemsep=0pt, parsep=1pt]
\item Remove apostrophe's from plural acronyms / initialisms, e.g.\ FPGA's, VMM's ASIC's, L1DDC's, ROC's, BC's, FIFO's  etc.
%\item convert '\textasciitilde' to '\textbackslash,'
%\item "e.g. " to "e.g.\textbackslash "
%\item front end and Front end to Front-end for NSW front-ends or front-end for a generic front-end.
%\item de-serialize  to deserialize
%\item ...ise to ...ize: serialise, ionise, max/minimise, digitise, realise, optimise, synchronise, multiplexer/multiplexor
%\item fanout to fan-out
%\item move the 40.079 MHz explanation to the overview. (from the ART section)
%\item change blank before cite, figure, table  to '\textbackslash,'
%\item Fig. to Figure
%\item sTDS to strip-TDS
%\item pTDS to pad-TDS
%\item miniSAS, to MiniSAS
%\item fanout to fan-out
\item {Pad Trigger: Is a hit map sent if the compression result would be bigger than the hit map?}
\end{itemize}
%Change ``USA15'' to ``radiation-protected room (USA15)''\\
}  % end red
